Extended Lagrangian approach for the numerical study of multidimensional dispersive waves: applications to the Serre-Green-Naghdi equations

In this paper we study two multidimensional nonlinear dispersive systems: the Serre-Green-Naghdi (SGN) equations describing dispersive shallow water flows, and Iordanskii-Kogarko-Wijngaarden (IKW) equations describing fluids containing small compressible gas bubbles. These models are Euler-Lagrange equations for a given Lagrangian and share common mathematical structure, namely the dependence of the pressure on material derivatives of macroscopic variables. We develop a generic dispersive model such that SGN and IKW systems become its special cases if only one specifies the appropriate Lagrangian, and then use the extended Lagragian approach proposed in Favrie and Gavrilyuk (2017) to build its hyperbolic approximation. The new approximate model is unconditionally hyperbolic for both SGN and IKW cases, and accurately describes dispersive phenomena, which allows to impose discontinuous initial data and study dispersive shock waves. We consider the 2-D hyperbolic version of SGN system as an example for numerical simulations and apply a second order implicit-explicit scheme in order to numerically integrate the system. The obtained 1-D and 2-D results are in close agreement with available exact solutions and numerical tests. \textbf{Keywords: } dispersive shallow water equations, bubbly fluids, Euler-Lagrange equations, hyperbolic conservation laws, multidimensional waves, implicit-explicit numerical methods

==> sections/abstract.tex <==
%\thispagestyle{empty}

\begin{center}
	{\large ANALYTICAL AND NUMERICAL STUDY OF A DISPERSIVE SHALLOW WATER MODEL}
\end{center}
\begin{center}
	\textbf{Abstract}
\end{center}

The present thesis is devoted to analytical and numerical modeling of nonlinear dispersive systems, notably Serre-Green-Naghdi equations (SGN equations) and Iordanskii-Kogarko-Wijngaarden bubbly fluids model (IKW model).  These models  share the common structure. First,  pressures of both models  depend on the material derivatives of their macroscopic variables. Second, SGN and IKW equations are the Euler-Lagrange equations coming from Hamilton's principle of stationary action, each one with its natural Lagrangian. Finally, the equations are Galilean invariant which is necessary for physically relevant mathematical models.

In the first part we derive the Whitham modulation equations for the SGN model and prove that these equations are strictly hyperbolic for any wave amplitude. We first obtain an exact periodic solution, the classical cnoidal wave, and then average the governing equations over its period to derive the Whitham modulation equations. Then, in order to get the explicit form of the equations, one should choose the set of variables to consider as primary. Our choice is not standard and does not necessarily have the physical sense, however it allows to reveal two symmetries of the system, which simplifies the hyperbolicity study: the original four-dimensional domain of study reduces to a two-dimensional  region, and eventually the hyperbolicity can be studied in a quadrant of a two-parameter plane.  Finally, we present a semi-analytical proof of the strict hyperbolicity of the Whitham system for SGN equations. This property can be interpreted by concluding that the periodic wave solutions of the SGN equations are modulationally stable. Numerical simulations of the full SGN equations are also shown, and these results confirm the theoretical stability results found by using the Whitham modulation theory.

In the second part, we derive and study a multi-dimensional  model which approximates both the SGN and IKW systems using the extended Lagrangian approach. This strategy relies on a fact that both models share the common structure and admit the variational formulation. Then we present the hyperbolicity study and  study of the eigenfields. The new approximate model is hyperbolic and accurately describes dispersive phenomena while possessing the properties of classic Euler equations, which allows to impose discontinuous initial data and study dispersive shock waves. We take the approximate  SGN system as an example for numerical simulations. Numerical tests for one- and two-dimensional  dispersive shock waves are presented. The results are in a good agreement with those obtained via existing numerical models of the exact SGN system.\\

\textbf{Keywords: } Dispersive shallow water equations, Euler-Lagrange equations, Whitham equations, hyperbolicity, multi-dimensional wave propagation.

\pagebreak
%\thispagestyle{empty}

\begin{center}
	{\large ÉTUDE ANALYTIQUE ET NUMÉRIQUE D'UN MODÈLE DISPERSIF DES EAUX PEU PROFONDES}
\end{center}
\begin{center}
	\textbf{Résumé}
\end{center}


Le présent manuscrit est dédié à la modélisation analytique et numérique des systèmes dispersifs non-linéaires, notamment les équations de Serre-Green-Naghdi (SGN) et le modèle du liquide à bulles de Iordanskii-Kogarko-Wijngaarden (IKW). Ces modèles partagent une structure commune. Tout d'abord, les pressions des deux modèles dépendent des dérivées matérielles de leurs variables macroscopiques. Ensuite, les équations de SGN et IKW sont les équations d'Euler-Lagrange qui viennent du principe d'Hamilton de l'action stationnaire, chacun avec son lagrangien naturel. Enfin, les équations sont invariantes par rapport à la transformation de Galilée, ce qui est nécessaire pour les modèles mathématiques physiquement pertinents.

Dans une première partie nous dérivons les équations de modulation de Whitham pour le modèle de SGN et nous montrons qu'elles sont strictement hyperboliques quelque soit l'amplitude d'onde. Nous obtenons d'abord une solution périodique exacte, l'onde cnoïdale classique, puis nous moyennons les équations de base sur sa période pour dériver les équations de modulation de Whitham. Ensuite, pour avoir une forme explicite des équations, on doit choisir l'ensemble des variables à considérer comme primaires. Notre choix n'est pas standard et n'a pas forcement de sens physique, mais il nous permet de révéler deux symétries du système, ce qui simplifie l'étude de l'hyperbolicité : le domaine quatre-dimensionnel original se réduit à une région deux-dimensionnelle et l'hyperbolicité peut éventuellement être étudié dans un quadrant du plan des deux paramètres. Finalement, nous présentons une preuve semi-analytique de l'hyperbolicité stricte du système de Whitham pour les équations de SGN. Cette propriété peut être interprétée par la conclusion que les solutions périodiques des équations de SGN sont modulationnellement stable. Les simulations numériques du système complet de SGN sont présentées, et ces résultats confirment les résultats théoriques obtenus.

Dans une seconde partie, nous dérivons et étudions un modèle multidimensionnel qui se rapproche des deux modèles SGN et IKW, en utilisant l'approche du lagrangien étendu. Cette stratégie se base sur le fait que les deux modèles partagent une structure commune et possèdent la formulation variationnelle. Ensuite, nous présentons l'étude de l'hyperbolicité ainsi que l'étude des champs propres. Le nouveau modèle approché est hyperbolique et décrit précisément les phénomènes dispersifs, et de plus il possède les propriétés des équations classiques d'Euler, ce qui permet d'imposer les conditions initiales discontinues et d'étudier les ondes de choc dispersifs. Nous considérons le système approché de SGN comme un exemple pour les simulations numériques. Les tests numériques pour les chocs dispersifs uni- et deux-dimensionnels sont présentés. Les résultats sont en bon accord avec ceux obtenus par des modèles numériques du système SGN exacte.\\

\textbf{Mots--clés :} Équations dispersives des eaux peu profondes, équations d'Euler-Lagrange, équations de Whitham, hyperbolicité, propagation des ondes multidimensionnelles.
